Nordic vaccination strategies face/off via age range comparative analysis on key indicators of COVID-19 severity and healthcare stress level

In this paper we analyze the impact of vaccinations on spread of the COVID-19 virus for different age groups. More specifically we examine the deployment of vaccines in the Nordic countries in a comparative analysis where we analyze factors such as healthcare stress level and severity of disease through new infections, hospitalizations, intensive care unit (ICU) occupancy and deaths. Moreover, we analyze the impact of the various vaccine types, vaccination rate on the spread of the virus in each age group for Denmark, Finland, Iceland, Norway and Sweden from the start of the vaccination period in December 2020 until the end of August 2021. We perform a three-fold analysis: i) frequency analysis of infections and vaccine rates by age groups, ii) rolling correlations between vaccination strategies, severity of COVID-19 and healthcare stress level and; iii) we also employ the epidemic Renormalization Group (eRG) framework. The latter is used to mathematically model wave structures, as well as the impact of vaccinations on wave dynamics. We further compare the Nordic countries with England. Our main results are the quantification of the impact of the vaccination campaigns on age groups epidemiological data, across countries with high vaccine uptake. The data clearly shows that vaccines markedly reduce the number of new cases and the risk of serious illness.

==> Todo.tex <==
number of infection and vaccination per age range - model with eRG
Fraction that goes to SIU
Less viral charge to spread if you have been infected
Finish figures
Reinfection rate of vaccinated people
Infections leaking into Iceland
Vaccination strategies
Now you're vaccinated, then what - look at UK

==> links.tex <==
Vaccination strategies in Europe, down to country level:
https://www.ecdc.europa.eu/sites/default/files/documents/Overview-implementation-COVID-19-vaccination-strategies-vaccine-deployment-plans.pdf

Vaccine tracker for europe:
https://vaccinetracker.ecdc.europa.eu/public/extensions/COVID-19/vaccine-tracker.html#uptake-tab



==> todolist.tex <==
\section*{To do list:}

\begin{itemize}
    \item Complete analysis of correlations for UK & nordic countries [Nattapat].
    \item Use eRG to model the number of infections per age group, including the effect of vaccinations [Corentin].
    \item Explore re-infection rate for vaccinated individuals. Summarise literature and include in discussion together with comparison of our correlations.
    \item Define optimal vaccination strategies: is there a way to do that?
    \item stopping certain vaccines
    \item make a table with decisions
    \item Recommendations. What can we learn
    \item centralized vs decentralized
    \item Pay for testing
\end{itemize}

which vaccines are banned
delay between 1st and 2nd dose
strategy respect to age
